How Large a Vocabulary Does Text Classification Need? A Variational Approach to Vocabulary Selection

With the rapid development in deep learning, deep neural networks have been widely adopted in many real-life natural language applications. Under deep neural networks, a pre-defined vocabulary is required to vectorize text inputs. The canonical approach to select pre-defined vocabulary is based on the word frequency, where a threshold is selected to cut off the long tail distribution. However, we observed that such simple approach could easily lead to under-sized vocabulary or over-sized vocabulary issues. Therefore, we are interested in understanding how the end-task classification accuracy is related to the vocabulary size and what is the minimum required vocabulary size to achieve a specific performance. In this paper, we provide a more sophisticated variational vocabulary dropout (VVD) based on variational dropout to perform vocabulary selection, which can intelligently select the subset of the vocabulary to achieve the required performance. To evaluate different algorithms on the newly proposed vocabulary selection problem, we propose two new metrics: Area Under Accuracy-Vocab Curve and Vocab Size under X\% Accuracy Drop. Through extensive experiments on various NLP classification tasks, our variational framework is shown to significantly outperform the frequency-based and other selection baselines on these metrics.

==> NAACL2019 - Variational Vocabulary Reduction/compare.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[thb]
\small
\centering
\begin{tabular}{llllll} 
\toprule
Task                  & Acc & \#Param & Comp & \#Vocab & Time  \\
\midrule
\multirow{3}{*}{Snips}  & 96.1  & 760K  &1x & 11K     & 1.6s  \\
                                         & 95.8     & 210K  & 3x & 2K      & 1.5s  \\
                                         & 95.6     & 88K   & 9x & 100    & 1.3s  \\ 
\midrule
\multirow{3}{*}{AG-news}  & 91.4  & 16M  & 1x & 61K   & 2.1s  \\
                     & 91.4     & 2.8M  & 6x  & 10K & 1.5s  \\
                     & 90.1     & 0.8M  & 200x  & 2K & 1.1s  \\
\midrule
\multirow{3}{*}{SNLI} & 85.5     & 16M   & 1x & 42K     & 6.0s  \\
                      & 85.5     & 6.6M  & 2x & 10K    & 5.6s \\
                      & 83.9     & 4.2M  & 4x & 2K    & 5.2s  \\ 
\bottomrule
\end{tabular}
\caption{We list the memory consumption, inference speed and accuracy under different vocabulary budget for different NLP end tasks.}
\label{tab:compare}
\end{table}

==> NAACL2019 - Variational Vocabulary Reduction/datasets.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table*}
\small
\centering
\begin{tabular}{llllll} 
\toprule
Datasets & Task                                                                                               & Description                              & \#Class & \#Train & \#Test  \\
\midrule
ATIS-flight~\cite{tur2010left} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}NLU\end{tabular}}  & Classify Airline Travel dialog           & 21      & 4,478   & 893     \\
Snips~\cite{DBLP:journals/corr/abs-1805-10190}       &                         & Classify inputs to personal voice assistant & 7       & 13,084  & 700     \\
\midrule
AG-news~\cite{zhang2015character}     &  \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}DC\end{tabular}}  & Categories: World, Sports, etc  & 4 & 120,000 & 7,600   \\
DBPedia~\cite{lehmann2015dbpedia}     &                      & Categories: Company, Athlete, Album, etc & 14      & 560,000 & 70,000  \\
Sogou-news~\cite{zhang2015character}  &                         & Categories: Sports, Technology, etc      & 5       & 450,000 & 60,000  \\
Yelp-review~\cite{zhang2015character} &                         & Categories: Review Ratings (1-5)         & 5       & 650,000 & 50,000  \\ 
\midrule
SNLI~\cite{DBLP:conf/emnlp/BowmanAPM15}        &  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}NLI\end{tabular}}                   & Entailment: Contradict, Neutral,Entail   & 3       & 550,152 & 10,000  \\
MNLI~\cite{DBLP:conf/naacl/WilliamsNB18}        & & Multi-Genre Entailment   & 3       & 392,702 & 10,000  \\
\bottomrule
\end{tabular}
\caption{An overview of different datasets under different classification tasks including description and sizes.}
\label{tab:dataset}
\end{table*}

==> NAACL2019 - Variational Vocabulary Reduction/results.tex <==
\begin{table*}[thb]
\centering
\small
\begin{tabular}{lcclccc} 
\toprule
Datasets / Reported Accuracy         & Accuracy & Vocab                & Methods             & AUC         & Vocab@-3\% & Vocab@-5\%  \\ 
\midrule
\multirow{4}{*}{Snips / 96.7~\cite{DBLP:conf/interspeech/LiuL16}} & 95.9       &  \multirow{4}{*}{11000} & Frequency       &  77.4    & 81         & 61          \\
                       & 95.9       &                        & TF-IDF           &   77.6   & 81           & 62          \\
                       & 95.6       &                        & Group Lasso       &   82.1   & 77           & 52\\
                       & 96.0 &                        & VVD & \textbf{82.5}  & \textbf{52}  & \textbf{36}         \\ 
\midrule
\multirow{4}{*}{ATIS-Flight / 94.1~\cite{goo2018slot}}  & 93.8       &  \multirow{4}{*}{724}    & Frequency      &  70.1   & 33           & 28    \\
                       & 93.8       &                        & TF-IDF           &  70.5  & 34          & 28\\
                       & 93.8       &                        & Group Lasso      &  72.9  & 30           & 26\\
                       & 94.0       &                        & VVD & \textbf{74.8}  & \textbf{29}  & \textbf{26}  \\
\midrule
\midrule
\multirow{5}{*}{AG-news / 91.1~\cite{zhang2015character}}     & 91.6       &     \multirow{4}{*}{61673} & Frequency    &  67.1 &    2290        & 1379\\
                             & 91.6       &                        & TF-IDF          &     67.8    &    2214     &    1303 \\

                             & 91.2       &                        & Group Lasso         &  68.3   &    1867     &  1032 \\
                             & 91.6       &                        & VVD & \textbf{70.5}  &  \textbf{1000}  & \textbf{673}   \\ 
\midrule
\multirow{4}{*}{DBPedia / 98.3~\cite{zhang2015character}}     & 98.4       &  \multirow{4}{*}{563355} & Frequency          &  69.7 &    1000    & 743            \\
                             & 98.4       &                        & TF-IDF           &   71.7    & 1703           & 804      \\

                             & 97.9       &                        & Group Lasso         &     71.9   &     768        &    678        \\
                             & 98.5       &               & VVD & \textbf{72.2}  & \textbf{427}   & \textbf{297}   \\ 
\midrule
\multirow{4}{*}{Sogou-news / 95.0~\cite{zhang2015character}}  & 93.7       & \multirow{4}{*}{254495}  & Frequency     & 70.9  & 789 & 643 \\
                             & 93.7       &                        & TF-IDF           & 71.3    & 976  &  776      \\
                             & 93.6       &                        & Group Lasso      & 73.4  &  765 &  456 \\
                             & 94.0       &                        & VVD & \textbf{75.5}  & \textbf{312}   & \textbf{196}   \\ 
\midrule
\multirow{4}{*}{Yelp-review / 58.0~\cite{zhang2015character}} & 56.3       &    \multirow{4}{*}{252712} & Frequency           &  74.0        &      1315      &     683        \\
                             & 56.3       &                        & TF-IDF           &     74.1      &     1630       &    754       \\

                             & 56.5       &                        & Group Lasso         &    75.4       &  934       &     463     \\
                             & \textbf{57.4}       &                        & VVD & \textbf{77.9}      & \textbf{487} & \textbf{287}   \\
\midrule
\midrule
\multirow{4}{*}{SNLI / 86.7~\cite{DBLP:conf/naacl/WilliamsNB18}} & 84.1     &  \multirow{4}{*}{42392} & Frequency           &   72.2   &   2139      &  1362 \\
                      & 84.1     &                        & TF-IDF              &  72.8    &    2132   &      1429 \\
                      & 84.6     &                        & Group Lasso         &  73.6    &    1712  &      1093 \\
                      & \textbf{85.5}     &                        & VVD & \textbf{75.0} & \textbf{1414} & \textbf{854}  \\
\midrule
\multirow{4}{*}{MNLI / 72.3~\cite{DBLP:conf/naacl/WilliamsNB18}} & 69.2     &  \multirow{4}{*}{100158} & Frequency           &   78.5   & 1758         &  952        \\
& 69.2     &                        & TF-IDF              &   78.7  &   1656      & 934 \\
& 70.1     &                        & Group Lasso         &   79.2    & 1466         &  711 \\
& \textbf{71.2}     &                        & VVD &  \textbf{80.1} &  \textbf{1323}  & \textbf{641} \\
\bottomrule
\end{tabular}
\caption{Experimental Results on various NLP tasks and datasets on the proposed metrics in~\autoref{sec:metrics}. Bold accuracy means the result is statistically significantly better than the competitors. }
\label{tab:result}
\end{table*}

==> NAACL2019 - Variational Vocabulary Reduction/toomuchembedding.tex <==
% \usepackage{booktabs}


\begin{table}[thb]
\small
\centering
\begin{tabular}{llllll} 
\toprule
\begin{tabular}[c]{@{}l@{}} Cutoff\\Freq. \end{tabular} & Vocab & \begin{tabular}[c]{@{}l@{}}Remain\\Vocab \end{tabular} & \#Emb & \#CNN & \begin{tabular}[c]{@{}l@{}}\#Emb \\Ratio\end{tabular}  \\ 
\midrule
1                                                       & 60K  & 100\%                                                  & 15M   & 0.36M & 97.6\%                                                 \\ 
\midrule
5                                                       & 40K   & 21.7\%                                                 & 10M   & 0.36M & 95.6\%                                                 \\ 
\midrule
10                                                      & 24K   & 13\%                                                   & 6M    & 0.36M & 94.3\%                                                 \\ 
\midrule
20                                                      & 14K   & 9.4\%                                                  & 3.5M  & 0.36M & 90\%                                                   \\ 
\midrule
100                                                     & 4K    & 2.7\%                                                  & 1M    & 0.36M & 73\%                                                   \\
\bottomrule
\end{tabular}
\caption{Illustration of the frequency-based vocabulary selection heuristic on a typical CNN-based document classification model (Section~\ref{sec:data_and_architecture}). \#Emb is the number of parameters in the word embedding matrix (256 dimensions), and \#CNN is that in the CNN model. }
\label{tab:embedding_ratio}
\end{table}

==> compare.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[thb]
\small
\centering
\begin{tabular}{llllll} 
\toprule
Task                  & Acc & \#Param & Comp & \#Vocab & Time  \\
\midrule
\multirow{3}{*}{Snips}  & 96.1  & 760K  &1x & 11K     & 1.6s  \\
                                         & 95.8     & 210K  & 3x & 2K      & 1.5s  \\
                                         & 95.6     & 88K   & 9x & 100    & 1.3s  \\ 
\midrule
\multirow{3}{*}{AG-news}  & 91.4  & 16M  & 1x & 61K   & 2.1s  \\
                     & 91.4     & 2.8M  & 6x  & 10K & 1.5s  \\
                     & 90.1     & 0.8M  & 200x  & 2K & 1.1s  \\
\midrule
\multirow{3}{*}{SNLI} & 85.5     & 16M   & 1x & 42K     & 6.0s  \\
                      & 85.5     & 6.6M  & 2x & 10K    & 5.6s \\
                      & 83.9     & 4.2M  & 4x & 2K    & 5.2s  \\ 
\bottomrule
\end{tabular}
\caption{We list the memory consumption, inference speed and accuracy under different vocabulary budget for different NLP end tasks.}
\label{tab:compare}
\end{table}
